Inference From Visible Information And Background Knowledge

We provide a wide-ranging study of the scenario where a subset of the relations in a relational vocabulary are visible to a user --- that is, their complete contents are known --- while the remaining relations are invisible. We also have a background theory --- invariants given by logical sentences --- which may relate the visible relations to invisible ones, and also may constrain both the visible and invisible relations in isolation. We want to determine whether some other information, given as a positive existential formula, can be inferred using only the visible information and the background theory. This formula whose inference we are concered with is denoted as the \emph{query}. We consider whether positive information about the query can be inferred, and also whether negative information -- the sentence does not hold -- can be inferred. We further consider both the instance-level version of the problem, where both the query and the visible instance are given, and the schema-level version, where we want to know whether truth or falsity of the query can be inferred in some instance of the schema.

==> gnftoaut/gnfautdecide.tex <==
\subsection{Optimized decidability of $\gnf$ via translation to automaton}

%As before, we have shown decidability of $\gnf$ via the tree model property
%and tree satisfiability. Now we will look for a more efficient procedure
%using automata.
We are now ready to translate $\gnf$ sentences to automata, and use this
to decide $\gnf$ satisfiability more efficiently.

We will build an automaton for a sentence $\varphi$ in $\gnf$ inductively,
so we will need to deal with formulas with free variables.
In order to deal with free variables,
the tree encodings
can be extended with additional information
about valuations for these variables.
Such trees use an extended signature.
Namely, for each free first-order variable $z$ and each $c \in \paramsk$,
we introduce a predicate $V_{c / z}$;
if $V_{c / z}(v)$ holds, then this indicates that the valuation for $z$
is the element named by $c$ at~$v$.
We refer to these additional predicates that give a valuation for the free variables
as \emph{free variable markers}.
In a valid tree code,
the free variables markers
for a first-order variable $z$
must satisfy the condition that there is a unique $v$ and unique $c \in \bagnames{v}$ such that
$V_{c / z}(v)$ holds
(i.e.~for each $z$ there is exactly one $V_{c/z}$-fact in the tree).
%The markers for a second-order variable $Y$
%must satisfy the condition that if
%$Y_{\vec{a}}(v)$ then $\vec{a} \subseteq \bagnames{v}$.

%\myparagraph{First attempt}

As a first attempt, we can proceed by induction on the structure of the formula
to build up an automaton $\autA_\phi$.

Starting with some atomic formula $R(x_1,\dots,x_n)$,
it is easy to construct an automaton
that checks that $R(x_1,\dots,x_n)$ holds
based on the valuations for the free variable markers for $x_1, \dots, x_n$.
The idea is that Eve has to navigate to a node where some $R(b_1,\dots,b_n)$ is in the label.
Adam can then challenge Eve to show that $\vec{x}$ corresponds to $\vec{b}$.
Say he challenges her on $b_i$.
Then Eve must navigate from $v$ to
the node carrying the marker $b_i/x_i$.
However, she must do this
by passing through a series of nodes
that also contain $b_i$.
If she is able to do this,
the automaton enters a sink state with priority 0, so Eve wins.

For the inductive cases, we then rely on the closure properties of $\ptwowayaltinf$.
For a conjunction or disjunction,
we can take the intersection or union, respectively, of the inductively defined automata for the
individual conjuncts or disjuncts.
For negation,
we take the automaton for the complement language.
Finally, for existential quantification,
we take the projection of the automaton on the appropriate free variable markers.

Proceeding in this fashion, we can build up an automaton $\autA_\phi$
for some $\phi \in \gnf$.
For instance, for $\phi$ a CQ, it would lead to an automaton with the following properties:
\begin{lemma}\label{lemma:autcq}
Given a CQ $\chi(x_1,\dots,x_j) = \exists \vec{y} ~ \eta(x_1,\dots,x_j,\vec{y}) $
of width at most $k$
over signature $\sigma'$,
we can construct a
$\ponewayndinf$ $\calN_{\chi}$
such that for all valid $k$ tree codes~$\tree$
with free variable markers $V_{a_1/x_1}(v_1),\dots,V_{a_j/x_j}(v_j)$,
\begin{align*}
&\text{$\calN_{\chi}$ accepts $\tree$} \quad
\text{iff} \quad \text{$\decode{T}$ satisfies $\chi([v_1,a_1],\dots,[v_j,a_j])$} .
\end{align*}

Furthermore, there is a polynomial function $g$ independent of~${\chi}$
such that the number of states of $\calN_{\chi}$
is at most $2^{g(k r_{\chi})}$
and the number of priorities is at most $g(k r_\chi)$
where
$r_{\chi}$ is the CQ-rank of~${\chi}$.
The overall size of the automaton
and the running time of the construction
is at most exponential in $\mysize{\sigma'} \cdot 2^{g(k r_{\chi})}$.
It is monotonic with respect to $\sigma'$.\footnote{
Recall the monotonicity property on page \pageref{def:monotonicity}.
We abuse the terminology slightly here,
and say the automaton $\calN_\chi$ over tree codes
is \emph{monotonic with respect to $\sigma'$}
if for all states $q$ in the state set of $\calN_\chi$
and for all $\tau' \subseteq \set{ P_{\vec{b}} : P \in \sigma'}$,
$\delta(q,\tau)$ entails $\delta(q,\tau \cup \tau')$.
Note that it easy to ensure monotonicity for the automaton for a CQ $\chi$:
if we had an automaton for the CQ $\chi$ with transition function $\delta$
that did not satisfy this monotonicity property,
then for each state $q$ and label $\tau$,
we could create a new transition function
$\delta'(q,\tau) := \delta(q,\tau) \vee \bigvee_{ \tau'' \subseteq \set{P_{\vec{b}} : P \in \sigma'}} \delta(q,\tau \setminus \tau'' )$.
Because of the positivity of the relations in $\sigma'$ in $\chi$,
it is easy to check that this would still result in an automaton for $\chi$.}
\end{lemma}

This approach just naively applying the closure properties of $\ptwowayaltinf$ is fine
for constructing an automaton for a CQ or a UCQ.
But it leads to large automata when we start nesting UCQs using guarded negation,
since we get an exponential blow-up in the size of the state set every time we need to do a projection.
Indeed, this approach does not get us any better bound than the approach
via logic and Rabin's theorem---it would still lead to a satisfiability algorithm of non-elementary complexity.

It turns out that we can do much better.

%\myparagraph{Improved construction using localization}
In the improved construction of $\autA_\phi$,
we assume that $\phi$ is in \nf, and
we will proceed by induction on the negation depth of $\phi$.

In order to avoid an exponential blow-up for each level of nesting,
we take advantage of the fact that the nesting of UCQs
allowed in $\gnf$ is restricted:
the free variables in a nested UCQ-shaped formula
must be guarded,
and hence must be represented locally
in a single node in the tree code.
Recall that a UCQ-shaped formula in $\gnf$ with negation depth greater than 0 is of the form
$\delta[Y_1 := \alpha_1 \wedge \neg \psi_1, \dots , Y_s := \alpha_s \wedge \neg \psi_s]$
where $\delta$ is a UCQ over the extended signature $\sigma'$ obtained from
$\sigma$ by adding fresh relations $Y_1, \dots, Y_s$,
each $\psi_i$ is a UCQ-shaped formula in $\gnf$,
and each $\alpha_i$ is a guard in $\sigma$ for the free variables of $\psi_i$.
We first construct an automaton for $\delta$, over the extended signature $\sigma'$.
The automaton for $\delta[Y_1 := \alpha_1 \wedge \neg \psi_1, \dots , Y_s := \alpha_s \wedge \neg \psi_s]$ can then
simulate the automaton for $\delta$
while allowing Eve to guess the valuations
for each $Y_i$ (i.e.~valuations for
each subformula $\alpha_i \wedge \neg \psi_i$).
In order to prevent Eve from cheating
and just guessing that every tuple satisfies these subformulas,
Adam is allowed to challenge her on these guesses
by launching an inductively defined automaton for these subformulas.

The technical difficulty here is that the free variable markers for these
subformulas are not written on the tree code any more---they are being guessed on-the-fly by Eve.
In order to cope with this, the inductive process will construct an
automaton for $\psi$
that can be launched from some internal node $v$ in the tree 
to test whether $\psi$ holds with a valuation $[v,\vec{a}]$ for $\vec{x}$.
The automaton will not specify a single initial state.
Instead,
there will be a designated initial state for each
possible ``local assignment''
for the free variables $\vec{x}$.
A \emph{local assignment} $\vec{a}/\vec{x}$
for $\vec{a} = a_1 \dots a_n \in \paramsk^n$ and $\vec{x} = x_1 \dots x_n$ is a mapping
such that $x_i \mapsto a_i$.
A node $v$ in a valid tree code $\tree$ with $\vec{a} \subseteq \bagnames{v}$
and a local assignment $\vec{a}/\vec{x}$,
specifies a valuation for $\vec{x}$.
We say it is local since the free variable markers for $\vec{x}$
would all appear locally in $v$.

We will write $\cA_\psi$ for the automaton for $\psi$
(without specifying the initial state),
and will write $\cA_\psi^{\vec{a}/\vec{x}}$ for $\cA_\psi$
with the designated initial state for $\vec{a}/\vec{x}$.
We call $\cA_\psi$ a \emph{localized automaton for $\psi$},
since when it is launched from a node $v$
from the designated initial state for $\vec{a}/\vec{x}$,
it is testing whether $\psi$ holds when the valuation for $\vec{x}$ is
$[v,\vec{a}]$, which is represented locally at $v$.
The point of localized automata is that they can test
whether a tuple of elements that appear together in a node satisfy some
property, but without having the markers for this tuple explicitly written on the
tree. In particular, we will use this for testing \emph{answer-guarded subformulas}:
formulas $\phi$ that are logically equivalent to $R(\vec{x}) \wedge \phi$
where $R(\vec{x})$ is a guard for the free variables in $\phi$.

\begin{lemma}\label{lemma:localsubstitution}
Let $\eta$ be in $\gnf$ over $\sigma \cup \set{Y_1,\dots,Y_s}$
that is positive in $Y_1,\dots,Y_s$.
Let $\cA_\eta$ be a localized $\ptwowayaltinf$ for $\eta$
over $\sigcode{\sigma \cup \set{Y_1,\dots,Y_s}}{k}$-trees
that is monotonic with respect to $Y_1,\dots,Y_s$.

For $1 \leq i \leq s$, let $\chi_i(\vec{z}_i)$ be an answer-guarded formula in $\gnf$ over $\sigma$
with the number of free variables in $\chi_i$ matching the arity of $Y_i$,
and let $\cA_{\chi_i}$ be a localized $\ptwowayaltinf$ for $\chi_i$
over $\sigcode{\sigma}{k}$-trees.

Then we can construct a localized $\ptwowayaltinf$ $\cA_{\psi}$ over
$\sigcode{\sigma}{k}$
for $\psi := \eta[Y_1 := \chi_1,\dots,Y_s := \chi_s]$
in linear time
such that the number of states (respectively, priorities) is at most
the sum of the number of states (respectively, priorities)
in $\cA_\eta$, $\cA_{\chi_1}, \dots, \cA_{\chi_s}$.
\end{lemma}


Using the previous lemma, we can construct the desired automaton
by induction on the negation depth of the formula.

\begin{lemma}\label{lemma:aut}
Given a $\nf$ formula $\psi(\vec{x})$ in $\gnf$ of width at most $k$ over signature $\sigma$,
we can construct a
$\ptwowayaltinf$ $\calA_\psi$
such that for all valid $k$ tree codes $\tree$,
for all local assignments $\vec{a}/\vec{x}$,
and for all nodes $v$ in $\tree$ with $\vec{a} \subseteq \bagnames{v}$,
\begin{align*}
&\text{$\calA_\psi^{\vec{a}/\vec{x}}$ accepts $\tree$
starting from $v$} \quad
\text{iff} \quad \text{$\decode{T}$ satisfies $\psi([v,\vec{a}])$} .
\end{align*}

Further, there is a polynomial function $f$ independent of~$\psi$
such that the number of states of $\calA_\psi$
is at most $N_\psi := f(m_\psi) \cdot 2^{f(k r_\psi)}$
and the number of priorities is at most $f(k m_\psi)$
where $m_\psi = \mysize{\psi}$, 
$r_\psi$ is the CQ-rank of~$\psi$.
The overall size of the automaton
and the running time of the construction
is at most exponential in $\mysize{\sigma} \cdot N_\psi$.
\end{lemma}

By combining this with an automaton that checks that
the input tree is a valid $k$ tree code,
we can test satisfiability of sentences from $\gnf$ in $\twoexptime$.

\begin{theorem} \label{thm:gnftwoexp} There is a $\twoexptime$ procedure
that decides satisfiability of $\gnf$ formulas.
\end{theorem}

With a little more effort,
we could even show that we can construct a $\btwowayaltinf$ for $\psi$ in $\gnf$,
but this is not important for achieving the $\twoexptime$ bound on satisfiability.

\input{gnfautdecidespecializations}


==> gnftoaut/lecnotesmacros.tex <==
\newcommand{\sourcea}{\kw{Sourcea}}
\newcommand{\sourceb}{\kw{Sourceb}}
\newcommand{\targetb}{\kw{Targetb}}
\newcommand{\targeta}{\kw{Targeta}}

\newcommand{\sqltorc}{\kw{SQLToRC}}
\newcommand{\sqlsq}{\kw{SQL}_{\kw{Subquery}}}
\newcommand{\sqlbs}{\kw{SQLBasSel}}
\newcommand{\usqlbs}{\kw{USQLBasSel}}
\newcommand{\pra}{\kw{RA^+}}
\newcommand{\pefo}{\exists FO^+}
\newcommand{\distinct}{\kw{DISTINCT}}
%\newcommand{\select}{\kw{SELECT}}
\newcommand{\swhere}{\kw{WHERE}}
\newcommand{\sfrom}{\kw{FROM}}
\newcommand{\sand}{\kw{AND}}
\newcommand{\sor}{\kw{OR}}
\newcommand{\compose}{\circ}
\newcommand{\prc}{RC^+}
\newcommand{\relop}{\kw{RelOp}}

\newcommand{\visitingstud}{\kw{VisitingStudent}}
\newcommand{\ptstud}{\kw{PartTimeStudent}}

\newcommand{\guestlecture}{\kw{GuestLecture}}
\newcommand{\guestname}{\kw{GuestName}}
\newcommand{\ldate}{\kw{LectureDate}}
\newcommand{\lecturername}{\kw{LecturerName}}
\newcommand{\homeinst}{\kw{HomeInstitution}}

\newcommand{\er}{\kw{ER}}
\newcommand{\cardcon}{\kw{CardConstr}}
\newcommand{\partwhole}{\kw{PartWhole}}
\newcommand{\subclass}{\kw{IsA}}
\newcommand{\mypw}{\partwhole}
\newcommand{\mysub}{\subclass}
\newtheorem{theorem}{Theorem}
\newtheorem{proposition}{Proposition}
\newtheorem{example}{Example}
%\newtheorem{proof}{Proof}
%


\newcommand{\numpart}{\kw{NumberParts}}
\newcommand{\numsub}{\kw{NumberSubClasses}}
\newcommand{\tableof}{\kw{TableOf}}
\newcommand{\tupleof}{\kw{TupleOf}}
\newcommand{\translateinst}{\kw{TranslateInst}}
\newcommand{\translateschema}{\kw{TranslateSchema}}
\newcommand{\erstruct}{\kw{S}}

\newcommand{\relinst}{\kw{I}}


\newcommand{\adomrc}{\kw{ADomRC}}
\newcommand{\adomrcnc}{\adomrc^-}
\newcommand{\rc}{\kw{RC}}
\newcommand{\ra}{\kw{RA}}
\newcommand{\sch}{\kw{S}}
\newcommand{\adomra}{\kw{AdomToRa}}
\newcommand{\ratoadom}{\kw{RaToAdom}}
\newcommand{\rctoadom}{\kw{SafeRcToAdom}}
\newcommand{\place}{\kw{Pl}}
\newcommand{\erase}{\kw{Erase}}
\newcommand{\rop}{\kw{RelOp}}
\newcommand{\seman}{\kw{Eval}}
\newcommand{\qadom}{\kw{GetAdomQ}}
\newcommand{\ER}{\kw{ER}}
\newcommand{\card}{\kw{CARD}}
%\newcommand{\partwhole}{\kw{Part-Whole}}
%\newcommand{\subclass}{\kw{Subclass}}

\newcommand{\source}{\kw{Source}}
\newcommand{\target}{\kw{Target}}
\newcommand{\prof}{\kw{Professor}}
\newcommand{\major}{\kw{StudMajor}}
\newcommand{\course}{\kw{Course}}
\newcommand{\courseid}{\kw{Courseid}}
\newcommand{\enroll}{\kw{Enrollment}}
\newcommand{\coursename}{\kw{Coursename}}
\newcommand{\hastaken}{\kw{HasTaken}}
\newcommand{\yeartaken}{\kw{YearTaken}}
\newcommand{\cyear}{\kw{Year}}
\newcommand{\term}{\kw{Term}}
\newcommand{\age}{\kw{Age}}
\newcommand{\fname}{\kw{FirstName}}

\newcommand{\const}[1]{\kw{Const}(#1)}
\newcommand{\raunion}{\kw{UNION}}

\newcommand{\schema}{\kw{Schema}}

\newcommand{\<}{\langle}
\renewcommand{\>}{\rangle}

\newcommand{\vdom}{\kw{Type}}

\newcommand{\mvbeat}[1]{}

\renewcommand{\state}[1]{\textstyle \langle #1 \rangle}
\newcommand{\specializations}[1]{\kw{Spec}(#1)}
\newcommand{\clgnf}[1]{\kw{cl}_{\kw{GN}}(#1)}

